Routing-Aware Partitioning of the Internet Address Space for Server Ranking in CDNs

The goal of Content Delivery Networks (CDNs) is to serve content to end-users with high performance. In order to do that, a CDN measures the latency on the paths from its servers to users and then selects a best available server for each user. For large CDNs, monitoring paths from thousands of servers to millions of users is a challenging task due to its size. In this paper, we address this problem and propose a framework to scale the task of path monitoring. Simply stated, the goal of our framework is clustering IP addresses (clients) such that in each cluster the choice of best available server is same (or similar). Then, finding a best available server for one client in a given cluster will be sufficient to assign that server to the rest of the clients in the cluster. To achieve this goal, first we introduce two distance metrics to compute how similar the server choices of any given two clients. Second, we use a clustering method that is based on interdomain routing information. We evaluate the goodness of our clusters by using the metrics we introduce. We show that there is a strong correlation between the similarity in how two destination clients are routed to in the Internet and the similarity in their server selections. Finally, we show how to choose representative clients from each cluster so that it is sufficient to learn the latencies from the CDN servers to the representative and find a best available server accordingly for the rest of the clients in the same cluster.

==> info.tex <==

To motivate the topic of ping point quality and coverage, consider that the mapping system clusters high load name servers and uses a single ping point to represent the group for measurements. This strategy is used for a few reasons. Not every name server is pingable, and hence we can't measure performance to all name servers. Furthermore, there are too many active client resolvers making it practically impossible to cluster every one of them. And finally, the mapping system would not scale well at various levels if it weren't for this grouping. However, the selection of a ping point for a cluster may be imperfect, thus impacting the quality of the performance measurements made by the mapping system. In this document, we name the problems caused by the aforementioned points as ?ping point quality and coverage problems?.
The mapping system depends on rudimentary metrics such as latency and loss measurements from ICMP pings. Furthermore, Mapping Engineering is evaluating different approaches that might improve the scoring systems ability to predict performance. Regardless of the measurements used, these measures can?t be 100\% reliably predictive for a variety of reasons. For instance, with respect to ICMP, ping budget limits are necessary in order to play nice with network providers. As a result, these measurements offer weak statistical estimators of real network conditions. Furthermore, the scoring function applied to the latency and loss estimators cannot simultaneously be a good predictor of throughout for long lived connections and for latency of small transactions. As a result, some information is lost in the aggregation, and the combination may not reflect the real transactional performance expectations for a set of end­users. There are also many ?corner? cases where ICMP pings get unfair treatment as the other higher­layer protocol packets, and therefore completely invalidate the scoring metrics. No scoring mechanism is going to be a good fit for every application, but it is useful to get a sense of how predictive different measurement strategies are. In this document, we refer to metrics that capture how predictive a scoring strategy is as ?scoring quality? metrics.
And finally, our mapping system is also instrumented to serve maprules from a partial set of our regions and deployments in the name of efficiency (to reduce COGS, promote better hit rates, etc.). ?Mapping operations? makes decisions about where to allocate capacity in order to meet performance objectives while reducing costs. We rely on techniques such as linear programming, capacity planning, traffic engineering (e.g. playing with maprule priorities), and manual adjustments, etc. to optimize our cost of operations (COGS) and adapt to requirements from our network partners/customers. As a result, sometimes ?Mapping Operations? intentionally (or unintentionally) makes capacity allocation decisions that cause the mapping system to direct traffic to places that might not meet performance objectives. We classify the problems caused by these issues as ?maprule QoS? problems.


PING POINT QUALITY

Assigning a ping point is equivalent to clustering the address space. If end­users with different performance measurements to our ecors are clustered together, it is not possible to find a single proxy for them all. The clustering is currently done by TCM/CPD and then MPD. TCM/CPD takes only as input the traceroute data from tracer regions to nameservers as seen in Swan logs. MPD then breaks or merges clusters generated by CPD. This methods has some fundamental
issues: . Tracing to NS limits the ping point coverage to only highly populated NS address, not necessarily all end­user address space of interests.
2. Choosing ping point only from routing path may eliminate possibly good ping point that is only one hop further.
3. Even with sufficient traceroute data, the current algorithm tries to maximize covered NS demand, which may underlook the coverage of end­user space.
4. There is an upper bound on the number of ping points due to the relation with MPD and the limit on the number of MPGs.
5. MPD may even eliminate Ping Points CPD assigned by merging clusters generated by CPD.
All these factors could contribute to bad ping point coverage in some geographical locations, or for some end­user networks. The challenges lie in how we can detect any deficiency in the system
Challenges on Ping Point Coverage. We first need to be able to tell if we are covering well the Internet space using ping points. We need to answer the following questions:
1. What are the interested Internet address space we need a good ping point coverage?
2. Are the current ping budget enough to cover all the interested end­user address space?
Are there even any redundancy in the current ping point selection?
3. What kind of expectation we should set for each separate end­user population?
4. How are we going to measure the ping point coverage, alert against the expectation and
react to it?
Challenges on Point Point Quality Metric. A good ping point can predict the end­user?s performance very well. Assuming we have the perfect scoring function, then the quality is solely based on whether the measurement on a ping point is a good estimation of the same measurement to the end­users. The difficulties of doing so are as follows:
1. We may compare these two different measurement directly. But either ping or traceroute data to end­user population is difficult to obtain. One reason is that end­user space is much larger but most are not as responsive as NS space.
2. Can we tell a bad ping point from good ones from the Ping Point measurement itself? What are the potential attributes that makes good ping point?
3. Client­NS association adds to another layer of difficulty. A good Ping point for a NS is not necessarily good for the underlying end­users because end­users may use a NS that is far away or close but not on the same routing path to our ecors.
4. Given a good quality metric, can we suggest a better Ping Point with the limited data we have, which may result in some manual ping point configurations?



Cluster validity is a fragile concept. There have been a dozen proposals, but none that is truly convincing.

I recommend to use an application for evaluation.

Only if the clustering helps you solve an actual problem then it was successful. It's meaningless to score high on some artificial metric if you can't apply it to real problems.




This allows Akamai to adjust its map, which determines which clients are directed to which regions, on this time scale. 
One obvious concern is that network conditions can change rapidly, and changing the location to which an end user is mapped only once every half hour may not be fast enough. 

==> ranking-servers.tex <==
1. The references that are pointed by the reviewers are added. Their relation with our work is decribed.

- Michael J. Freedman, Mythili Vutukuru, Nick Feamster, Hari Balakrishnan: Geographic Locality of IP Prefixes. Internet Measurement Conference 2005: 153-158
- Bamba Gueye, Steve Uhlig, Serge Fdida: Investigating the Imprecision of IP Block-Based Geolocation. PAM 2007: 237-240
- Ingmar Poese, Steve Uhlig, Mohamed Ali Kâafar, Benoit Donnet, Bamba Gueye: IP geolocation databases: unreliable? Computer Communication Review 41(2): 53-56 (2011)
- Improving Content Delivery with PaDIS" IMC 2010, 
- Enabling Content-aware Traffic Engineering,  ACM SIGCOMM CCR 2012.
- End-User Mapping: Next Generation Request Routing for Content Delivery, 2015

